Exploring Continual Fine-Tuning for Enhancing Language Ability in Large Language Model

A common challenge towards the adaptability of Large Language Models (LLMs) is their ability to learn new languages over time without hampering the model's performance on languages in which the model is already proficient (usually English). Continual fine-tuning (CFT) is the process of sequentially fine-tuning an LLM to enable the model to adapt to downstream tasks with varying data distributions and time shifts. This paper focuses on the language adaptability of LLMs through CFT. We study a two-phase CFT process in which an English-only end-to-end fine-tuned LLM from Phase 1 (predominantly Task Ability) is sequentially fine-tuned on a multilingual dataset -- comprising task data in new languages -- in Phase 2 (predominantly Language Ability). We observe that the ``similarity'' of Phase 2 tasks with Phase 1 determines the LLM's adaptability. For similar phase-wise datasets, the LLM after Phase 2 does not show deterioration in task ability. In contrast, when the phase-wise datasets are not similar, the LLM's task ability deteriorates. We test our hypothesis on the open-source \mis\ and \llm\ models with multiple phase-wise dataset pairs. To address the deterioration, we analyze tailored variants of two CFT methods: layer freezing and generative replay. Our findings demonstrate their effectiveness in enhancing the language ability of LLMs while preserving task performance, in comparison to relevant baselines.

==> tables/mitigation_la.tex <==
%
%%%
%%%%% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~`
\begin{table*}[t]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{ccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}}     & \textbf{Phase 1} & \textbf{Phase 2} & \textbf{Mitigating} & \multirow{1}{*}{\textbf{MLQA}}  & \multirow{1}{*}{\textbf{XLSum}} &  \multirow{1}{*}{\textbf{XQUAD}}   \\  
    & \textbf{Dataset} & \textbf{Dataset} & \textbf{Strategy} & & &   \\
    \midrule
    \multirow{6}{*}{\mis} & \multirow{6}{*}{Instruct} & -- &  -- &  0.246 & 0.012 &  0.351 \\
     &  & \multirow{5}{*}{\malp} &  -- & 0.307 & 0.033 & 0.436 \\
    & & & Layer Freezing \textbf{(H1)} & 0.176  & 0.016   &    \\  
                            & &  & Layer Freezing \textbf{(H2)} & 0.213 & 0.014 &  0.442  \\  
                             &  &  & Gen Replay \textbf{(H1)} &  0.311 & 0.008 & 0.428  \\  
                          &  &  &  Gen Replay \textbf{(H2)} &  0.213 & 0.007 & 0.427  \\  
                          &   &  &  \textcolor{green}{Replay} & &   &      \\
    \midrule
    \multirow{6}{*}{\llm} & \multirow{6}{*}{Instruct} & -- & -- & 0.609 & 0.0484 & 0.712  \\
     &  & \multirow{5}{*}{\malp} & -- & 0.321 & 0.0296 &  \\
    & & &  Layer Freezing \textbf{(H1)} & 0.368  & 0.037 & 0.505\\  
                          & &  & Layer Freezing \textbf{(H2)}  &  0.3995 & 0.038 & 0.505\\  
                          &  &  & Gen Replay \textbf{(H1)} & 0.437  & 0.019   & 0.593 \\  
                          & &  & Gen Replay \textbf{(H2)}  &   &  &   \\ 
                         &   &  &  \textcolor{green}{Replay} &  &  &    \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Mitigating Strategies: Language Ability}
    \label{tab:results_interventions_LA}
\end{table*}
%%%%% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%%%%
%%5


==> tables/mixture.tex <==
\begin{table*}[t]
    \centering
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{ccc|ccccc|cccc}
    \toprule
     \textbf{Model} & \multicolumn{2}{c|}{\textbf{Dataset Mixture}} & \texttt{IFEval} & \texttt{Alpaca Eval} & \texttt{MMLU} & \texttt{HellaSwag} & \textbf{Avg.} & \texttt{MLQA}  & \texttt{XQuAD} & \texttt{XLSUM} & \textbf{Avg.} \\
    \midrule
      \mis   & \alp  & \malp & 0.394 & 0.229 & 0.538  & 0.602 & 0.441 & 0.406 & 0.217 & 0.079 & 0.234 \\
      % \mis  & \orca  & \morca & 0.228 &  &  0.284 & 0.444 & - & 0.201 &  0.128    &  0.071 & 0.134 \\ ----> appendix
      \llm  & \alp & \malp  & 0.363 & 0.070  & 0.598 & 0.602 & 0.408  & \textbf{0.480} & 0.139  & 0.040 & 0.220 \\
      % \llm & \orca & \morca & 0.248  & 7.185  &  0.484  & 0.473 & - & 0.224  & 0.091  &  0.034 & 0.116\\
    \bottomrule
    \end{tabular}}
    \caption{Task and Language Ability when the LLMs are trained on the mixture of Phase 1 and Phase 2 Datasets. The first five columns represent Task Ability, while the last three represent Language Ability.}
    \label{tab:data_mixture_combined}
\end{table*}
